FULLER: Unified Multi-modality Multi-task 3D Perception via Multi-level Gradient Calibration

Multi-modality fusion and multi-task learning are becoming trendy in 3D autonomous driving scenario, considering robust prediction and computation budget. However, naively extending the existing framework to the domain of multi-modality multi-task learning remains ineffective and even poisonous due to the notorious modality bias and task conflict. Previous works manually coordinate the learning framework with empirical knowledge, which may lead to sub-optima. To mitigate the issue, we propose a novel yet simple multi-level gradient calibration learning framework across tasks and modalities during optimization. Specifically, the gradients, produced by the task heads and used to update the shared backbone, will be calibrated at the backbone's last layer to alleviate the task conflict. Before the calibrated gradients are further propagated to the modality branches of the backbone, their magnitudes will be calibrated again to the same level, ensuring the downstream tasks pay balanced attention to different modalities. Experiments on large-scale benchmark nuScenes demonstrate the effectiveness of the proposed method, eg, an absolute 14.4% mIoU improvement on map segmentation and 1.4% mAP improvement on 3D detection, advancing the application of 3D autonomous driving in the domain of multi-modality fusion and multi-task learning. We also discuss the links between modalities and tasks.

==> latex/tab/ablation.tex <==

% \begin{table}[t]
%     \centering
%     \caption{Ablation Study.\xd{add caption, what do first lines mean}}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{1pt}{1.0}
%     \begin{tabular}{@{}cc|cccc@{}}
%     \toprule
%         % Modality Grad. & Task Grad. &mAP &NDS &mIoU\\
%         Intra-gradient & Inter-gradient &mAP(\%) &NDS &mIoU(\%) &$\Delta_{\rm MTL}$(\%)\\
%         \midrule
%         \midrule
%         \multicolumn{5}{c}{\textit{det\_loss:seg\_loss=1:1}}\\
%         \midrule
%         &  &59.09 & 65.03 & 43.97\\
%         \checkmark & &59.51 &65.36 &45.01\\
%         &\checkmark & 57.07 &63.34 &59.46\\
%         \checkmark &\checkmark &60.47  &65.34  &58.35\\
%         \midrule
%         \midrule
%         \multicolumn{5}{c}{\textit{det\_loss:seg\_loss=1:5}}\\
%         \midrule
        
%         &  &59.79 & 65.46 & 55.65 \\
%         \checkmark &  &59.83 &65.31 &56.13\\
%         &\checkmark &56.94 &63.31  &59.84\\
%         \checkmark &\checkmark & 60.13 & 65.62 & 58.24\\
%         \midrule
%         \midrule
%         \multicolumn{5}{c}{\textit{det\_loss:seg\_loss=1:10}}\\
        
%         \midrule
%         &  &59.31 & 65.00 & 57.92\\
%         \checkmark & & 60.05 & 65.41 & 57.30\\
%         &\checkmark &58.17  &64.16 & 60.05\\
%         \checkmark &\checkmark & 59.85 &65.18 &59.20\\
% \bottomrule
%     \end{tabular}}
%     \label{tab:ablation}
% \end{table}

\begin{table}[t]
    \centering
    % \caption{Ablation Study of the proposed inter-gradient and intra-gradient calibration under three different initial states.}
    \caption{Ablation Study of the proposed inter-gradient and intra-gradient calibration with three different initial states.}
    \vspace{-0mm}
    \resizebox{1.0\columnwidth}{!}
    {\tablestyle{5pt}{1.0}
    \begin{tabular}{@{}cc|cccc@{}}
    \toprule
        % Modality Grad. & Task Grad. &mAP &NDS &mIoU\\
        Intra-grad. & Inter-grad. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
        &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
        \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:1}}\\ s
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:1}}\\
        \midrule
        &  &59.1 & 65.0 & 44.0 &18.3\\
        \checkmark & &59.5 &\textbf{65.4} &45.0 &16.9\\
        &\checkmark & 57.1 &63.3 &\textbf{59.5} &8.8\\
        \checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{5.4}\\
        
        \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:5}}\\
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:5}}\\
        \midrule
        &  &59.8 & 65.5 & 55.7 &8.0\\
        \checkmark &  &59.8 &65.3 &56.1 &7.8 \\
        &\checkmark &56.9 &63.3  &\textbf{59.8} &8.7 \\
        \checkmark &\checkmark & \textbf{60.1} & \textbf{65.6} & 58.2 &\textbf{5.7}\\
        
        \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:10}}\\
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:10}}\\
        \midrule
        &  &59.3 & 65.0 & 57.9 &7.0\\
        \checkmark & & \textbf{60.1} & \textbf{65.4} & 57.3 &6.5\\
        &\checkmark &58.2  &64.2 & \textbf{60.1} &6.7\\
        \checkmark &\checkmark & 59.9 &65.2 &59.2 &\textbf{5.3}\\
\bottomrule
    \end{tabular}}
    \label{tab:ablation}\vspace{-4mm}
\end{table}

==> latex/tab/big_table.tex <==
% \begin{table*}[h]
%     \centering
%     \caption{\textbf{Improving Baseline.} This is the baseline where det loss and seg loss are 1:1. This table is copied from Bevfusin(@mit). Please adjust it according to our settings. 
%     {\color{green}{(zj: FULLER is running)}}}
%     \begin{threeparttable}
%     \begin{tabular}{@{}l|ccccc@{}}
%     \toprule
%          \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& &\multicolumn{2}{c}{Det} &Seg \\ \cline{3-4}
%           &Modality &mAP &NDS &mIoU  \\
%           \midrule
%          PointPainting& C+L & 65.8 & 69.6 & -\\
%          MVP& C+L& 66.1 & 70.0 & -\\
%          FusionPainting & C+L &66.5 & 70.7 & - \\
%          AutoAlign & C+L & 66.6 & 71.7 & - \\
%          FUTR3D & C+L & 64.5 & 68.3 & - \\
%          TransFusion & C+L & 67.5 & 71.3 & - \\
%          BEVFusion & C+L & 68.5 & 71.4 & - \\
%          \midrule
%          PointPainting & C+L & - & - & 49.1 \\
%          MVP & C+L & - & - & 49.0 \\
%          BEVFusion & C+L & - & - & 62.7 \\
%          \midrule
%          BEVFusion$^{\dag}$\_Joint(shared BEV encoders) & C+L & - & 69.7 & 54.0\\
%          BEVFusion$^{\footnotemark[2]}$\_Joint( BEV encoders) & C+L & - & 69.9 & 58.4\\
%          Baseline$^{*}$ (upper bound) &C+L & 62.07 & 66.57 & 62.27\\
%          Baseline& C+L & 59.09 & 65.03 & 43.97\\
%          %Method 1 &\\
%          %Method 2 & \\
%          Fuller& C+L \\
%          \bottomrule
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[*] is single-task learning, served as upper bound. $^{\dag}$ balances loss weights manually.
%     \end{tablenotes}
% \end{threeparttable}
% \label{tab:baseline}
% \end{table*}


\begin{table*}[t]
    \centering
    \caption{Comparison to more methods.}
    \vspace{-0mm}
    \resizebox{2.0\columnwidth}{!}
    {\tablestyle{8pt}{1.0}
    \begin{threeparttable}

    \begin{tabular}{@{}l|cccc|ccc}
    \toprule
         % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& & & &\multicolumn{2}{c}{Det} &Seg \\ \cline{5-6}
          &Modality& VoxelSize & LiDAR &Image &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ \\
          \midrule
          \midrule
         \multicolumn{8}{c}{3D Detection}\\
          \midrule
         M$^2$BEV~\cite{xie2022m} & C & -&- & ResNeXt-101~\cite{Xie_2017_CVPR}&\cellcolor{blue!5}41.7 &\cellcolor{blue!5}47.0 & -\\
         BEVFormer~\cite{li2022bevformer} & C & -& -& ResNet101~\cite{He_2016_CVPR}&\cellcolor{blue!5}41.6 &\cellcolor{blue!5}51.7 & -\\
         PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L &0.075 &PointPillars &- &\cellcolor{blue!5}52.3 &\cellcolor{blue!5}61.3 &- \\
         CenterPoint~\cite{yin2021center} &L & 0.075&VoxelNet &- &\cellcolor{blue!5}59.6 &\cellcolor{blue!5}66.8 &- \\
         PointPainting$^{\ddag}$~\cite{vora2020pointpainting}& C+L&0.075 & PointPillars &- & \cellcolor{blue!5}65.8 &  \cellcolor{blue!5}69.6 & -\\
         MVP$^{\ddag}$~\cite{yin2021multimodal}& C+L & 0.075 &  VoxelNet & DLA-34& \cellcolor{blue!5}66.1 & \cellcolor{blue!5}70.0 & -\\
         FusionPainting~\cite{xu2021fusionpainting} & C+L & -&Cylinder3D~\cite{zhou2020cylinder3d} &HTCNet~\cite{Chen_2019_CVPR}&\cellcolor{blue!5}66.5 & \cellcolor{blue!5}70.7 & - \\
         AutoAlign~\cite{chen2022autoalign} & C+L &0.075 & CenterPoint & ResNet-50& \cellcolor{blue!5}66.6 & \cellcolor{blue!5}71.1 & - \\
         FUTR3D~\cite{chen2022futr3d} & C+L & 0.075& VoxelNet & ResNet-101& \cellcolor{blue!5}64.5 & \cellcolor{blue!5}68.3 & - \\
         TransFusion~\cite{bai2022transfusion} & C+L &0.075 & VoxelNet&DLA-34& \cellcolor{blue!5}67.5 & \cellcolor{blue!5}71.3 & - \\
         BEVFusion~\cite{liu2022bevfusion} & C+L &0.075 & VoxelNet&Swin-T &  \cellcolor{blue!5}68.5 & \cellcolor{blue!5}71.4 & - \\
         % Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.60} &\cellcolor{blue!5}\textbf{71.30}  &- \\
         % Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.07} &\cellcolor{blue!5}\textbf{66.57} &- \\
         Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.6} &\cellcolor{blue!5}\textbf{71.3}  &- \\
         Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.1} &\cellcolor{blue!5}\textbf{66.6} &- \\
         \midrule
          \midrule
         \multicolumn{8}{c}{BEV Map Segmentation}\\
          \midrule
         OFT$^{\ddag}$~\cite{roddick2018orthographic} &C  &- &- &ResNet-18 &- &- &\cellcolor{blue!5}42.1 \\
         LSS$^{\ddag}$~\cite{philion2020lift} &C  &- &- &EfficientNet-B0~\cite{tan2019efficientnet}&- &-&\cellcolor{blue!5}44.4 \\
         PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L & 0.1&- &PointPillars &- &- &\cellcolor{blue!5}43.8 \\
         CenterPoint$^{\ddag}$~\cite{yin2021center} &L &0.1  &VoxelNet &- &- &-  &\cellcolor{blue!5}48.6 \\
         PointPainting$^{\ddag}$~\cite{vora2020pointpainting} & C+L  &0.1& PointPillars & - &- &- & \cellcolor{blue!5}49.1 \\
         MVP$^{\ddag}$~\cite{yin2021multimodal} & C+L &0.1 & VoxelNet & DLA-34\cite{yu2018deep}  &- &- & \cellcolor{blue!5}49.0 \\
         BEVFusion~\cite{liu2022bevfusion} & C+L  &0.1 & VoxelNet&Swin-T & -&- & \cellcolor{blue!5}62.7 \\
         % Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.27} \\
         Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.3} \\
         \midrule
          \midrule
         \multicolumn{8}{c}{3D Detection + BEV Map Segmentation}\\
          \midrule
         BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (share) & C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}- & \cellcolor{blue!5}69.7 & \cellcolor{blue!5}54.0\\
         BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (sep) & C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}- & \cellcolor{blue!5}69.9 & \cellcolor{blue!5}58.4\\
         % Baseline$^{*}$ (upper bound) &C+L &D+S & 62.07 & 66.57 & 62.27\\
         % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.09} & \cellcolor{blue!5}\textbf{65.03} & \cellcolor{blue!5}\textbf{43.97}\\
         % Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.47} &\cellcolor{blue!5}\textbf{65.34}  &\cellcolor{blue!5}\textbf{58.35}\\
         % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.1} & \cellcolor{blue!5}\textbf{65.0} & \cellcolor{blue!5}\textbf{44.0}\\
         Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}59.1 & \cellcolor{blue!5}65.0 & \cellcolor{blue!5}44.0\\
         Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.5} &\cellcolor{blue!5}\textbf{65.3}  &\cellcolor{blue!5}\textbf{58.4}\\
         \bottomrule
    \end{tabular}
    % \begin{tablenotes}
    %     \footnotesize
    %     \item[$\dag$] means the multi-task result in BEVFusion\cite{liu2022bevfusion}. $^{\ddag}$ means re-implementation result in BEVFusion\cite{liu2022bevfusion}. `share' means multi-task heads share one BEV encoder to process the fused multimodal feature. `sep' means task heads have separate encoders.
    % \end{tablenotes}
\end{threeparttable}}
\vspace{-3mm}
\label{tab:more_comparison}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \caption{Comparison with benchmark. The upper two sub-tables are single task results while the bottom one is multi-task result.‘L’ and ‘C’ represent LiDAR and Camera, respectively. We treat single task result as our upper bound because multi-task will generally decrease the performance. Baseline means Fuller is naively trained where detection loss and segmentation loss are set to 1:1. `-' means inapplicable.
%     %\xd{can remove some old methods into appendix}
%     }\vspace{-3mm}
%     \resizebox{2.0\columnwidth}{!}
%     {\tablestyle{5pt}{1.0}
%     \begin{threeparttable}

%     \begin{tabular}{@{}l|cccc|cccc}
%     \toprule
%          % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& & & &\multicolumn{2}{c}{Det} &Seg \\ \cline{5-6}
%           &Modality& VoxelSize & LiDAR &Image &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ &$\Delta_{\rm MTL}$(\%)$\downarrow$\\
%           \midrule
%           \midrule
%          \multicolumn{9}{c}{3D Detection}\\
%           \midrule
%         %  M$^2$BEV~\cite{xie2022m} & C & -&- & ResNeXt-101~\cite{Xie_2017_CVPR}&\cellcolor{blue!5}41.7 &\cellcolor{blue!5}47.0 & -\\
%          BEVFormer~\cite{li2022bevformer} & C &- &- & ResNet101~\cite{He_2016_CVPR}& 41.6 & 51.7 & - &-\\
%         %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L &0.075 &PointPillars &- &\cellcolor{blue!5}52.3 &\cellcolor{blue!5}61.3 &- \\
%          CenterPoint~\cite{yin2021center} &L & 0.075&VoxelNet &- & 59.6 & 66.8 &- &-\\
%         %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting}& C+L&0.075 & PointPillars &- & \cellcolor{blue!5}65.8 &  \cellcolor{blue!5}69.6 & -\\
%          MVP$^{\ddag}$~\cite{yin2021multimodal}& C+L & 0.075 &  VoxelNet & DLA-34&  66.1 &  70.0 &- &-\\
%         %  FusionPainting~\cite{xu2021fusionpainting} & C+L & -&Cylinder3D~\cite{zhou2020cylinder3d} &HTCNet~\cite{Chen_2019_CVPR}&\cellcolor{blue!5}66.5 & \cellcolor{blue!5}70.7 & - \\
%         %  AutoAlign~\cite{chen2022autoalign} & C+L &0.075 & CenterPoint & ResNet-50& \cellcolor{blue!5}66.6 & \cellcolor{blue!5}71.1 & - \\
%          % FUTR3D~\cite{chen2022futr3d} & C+L & 0.075& VoxelNet & ResNet-101& \cellcolor{blue!5}64.5 & \cellcolor{blue!5}68.3 & - \\
%          TransFusion~\cite{bai2022transfusion} & C+L &0.075 & VoxelNet&DLA-34&  67.5 &  71.3 &- &-\\
%          BEVFusion~\cite{liu2022bevfusion} & C+L &0.075 & VoxelNet&Swin-T &   68.5 &  71.4 & - &-\\
%          % Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.60} &\cellcolor{blue!5}\textbf{71.30}  &- \\
%          % Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.07} &\cellcolor{blue!5}\textbf{66.57} &- \\
%          Fuller-det &C+L  &0.075 & VoxelNet&Swin-T &  67.6 & 71.3  &- &-\\
%          Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T &  \textbf{62.1} & \textbf{66.6} &- &-\\
%          \midrule
%           \midrule
%          \multicolumn{9}{c}{BEV Map Segmentation}\\
%           \midrule
%         %  OFT$^{\ddag}$~\cite{roddick2018orthographic} &C  &- &- &ResNet-18 &- &- &\cellcolor{blue!5}42.1 \\
%          LSS$^{\ddag}$~\cite{philion2020lift} &C  &- &- &EfficientNet-B0&- &-& 44.4 &-\\
%         %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L & 0.1&- &PointPillars &- &- &\cellcolor{blue!5}43.8 \\
%          CenterPoint$^{\ddag}$~\cite{yin2021center} &L &0.1  &VoxelNet &- &- &-  & 48.6 &-\\
%         %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting} & C+L  &0.1& PointPillars & - &- &- & \cellcolor{blue!5}49.1 \\
%          % MVP$^{\ddag}$~\cite{yin2021multimodal} & C+L &0.1 & VoxelNet & DLA-34\cite{yu2018deep}  &- &- & \cellcolor{blue!5}49.0 \\
%          BEVFusion~\cite{liu2022bevfusion} & C+L  &0.1 & VoxelNet&Swin-T & -&- &  62.7 &-\\
%          % Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.27} \\
%          Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - & \textbf{62.3} &-\\
%          \midrule
%           \midrule
%          \multicolumn{9}{c}{3D Detection + BEV Map Segmentation}\\
%           \midrule
%          BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (share) & C+L  &0.1 & VoxelNet&Swin-T & - &  69.7 &  54.0 &-\\
%          BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (sep) & C+L  &0.1 &VoxelNet&Swin-T &  - &  69.9 &  58.4 &-\\
%          % Baseline$^{*}$ (upper bound) &C+L &D+S & 62.07 & 66.57 & 62.27\\
%          % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.09} & \cellcolor{blue!5}\textbf{65.03} & \cellcolor{blue!5}\textbf{43.97}\\
%          % Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.47} &\cellcolor{blue!5}\textbf{65.34}  &\cellcolor{blue!5}\textbf{58.35}\\
%          Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T&  {59.1} &  {65.0} &  {44.0} & {33.6}\\
%          Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T & \textbf{60.5} & \textbf{65.3}  & \textbf{58.4} & \textbf{10.8}\\
%          \bottomrule
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[$\dag$] means the multi-task result in BEVFusion\cite{liu2022bevfusion}. $^{\ddag}$ means re-implementation result in BEVFusion\cite{liu2022bevfusion}. `share' means multi-task heads share one BEV encoder to process the fused multimodal feature. `sep' means task heads have separate encoders.
%     \end{tablenotes}
% \end{threeparttable}}
% \vspace{-3mm}
% \label{tab:baseline}
% \end{table*}

==> latex/tab/disjoint_ablation.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Verifying the proposed inter-gradient and intra-gradient calibration under disjoint dataset.}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{5pt}{0.5}
%     \begin{tabular}{@{}ccc|cccc@{}}
%     \toprule
%         Setting &Intra. & Inter. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
%         &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
%         \midrule
%         \multirow{2}{*}{\rotatebox{90}{Full}} & & &59.1 & 65.0 & 44.0 &36.6\\
%         &\checkmark & &59.5 &\textbf{65.4} &45.0 &33.8\\
%         & &\checkmark & 57.1 &63.3 &\textbf{59.5} &17.5\\
%         &\checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{10.8}\\
%         \midrule
%         \multirow{2}{*}{\rotatebox{90}{Dj.-bl.}} & & &\textbf{58.7} & 64.2 & 41.5 &42.5\\
%         &\checkmark &  &58.3 &\textbf{65.0} &42.4 &40.5 \\
%         & &\checkmark &57.4 &62.7  &\textbf{57.3} &21.5 \\
%         & \checkmark &\checkmark & 58.4 & 63.6 & 56.7 &\textbf{19.5}\\
%         \midrule
%         \multirow{2}{*}{\rotatebox{90}{Dj.-nm.}}& &&59.1 & 64.7 & 43.1 &38.5\\
%         &\checkmark & &\textbf{59.3} &\textbf{65.3}  &44.0  &35.8\\
%         & &\checkmark &57.4  &62.9 & 53.8 &26.8\\
%         & \checkmark &\checkmark & 58.9 &64.9 &\textbf{55.0} &\textbf{19.4}\\
% \bottomrule
%     \end{tabular}}
%     \label{tab:disjoint_ablation}
% \end{table}

\begin{table}[t]
    \centering
    \caption{Verifying the proposed inter-gradient and intra-gradient calibration under disjoint dataset.}
    \resizebox{1.0\columnwidth}{!}
    {\tablestyle{5pt}{0.9}
    \begin{tabular}{@{}ccc|cccc@{}}
    \toprule
        Setting &Intra. & Inter. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
        &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
        \midrule
        % \multirow{2}{*}{\rotatebox{90}{Full}} & & &59.1 & 65.0 & 44.0 &36.6\\
        % &\checkmark & &59.5 &\textbf{65.4} &45.0 &33.8\\
        % & &\checkmark & 57.1 &63.3 &\textbf{59.5} &17.5\\
        % &\checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{10.8}\\
        % \midrule
        
        \multirow{2}{*}{\rotatebox{90}{Dj.-bala.}} 
         % \multirow{4}{*}{balance} 
        & & &\textbf{58.7} & 64.2 & 41.5 &42.5\\
        &\checkmark &  &58.3 &\textbf{65.0} &42.4 &40.5 \\
        & &\checkmark &57.4 &62.7  &\textbf{57.3} &21.5 \\
        & \checkmark &\checkmark & 58.4 & 63.6 & 56.7 &\textbf{19.5}\\
        \midrule
        \multirow{2}{*}{\rotatebox{90}{Dj.-norm.}}
        % \multirow{4}{*}{normal}
        & &&59.1 & 64.7 & 43.1 &38.5\\
        &\checkmark & &\textbf{59.3} &\textbf{65.3}  &44.0  &35.8\\
        & &\checkmark &57.4  &62.9 & 53.8 &26.8\\
        & \checkmark &\checkmark & 58.9 &64.9 &\textbf{55.0} &\textbf{19.4}\\
\bottomrule
    \end{tabular}}
    \label{tab:disjoint_ablation}
\end{table}

==> latex/tab/mtl_result.tex <==
% \begin{table}
%   \centering
%   \caption{
%   % \xd{move to experiment as we have many analysis figures before method already} 
%   % We evaluate existing works of multi-task learning in our baseline. We empirically find that GradNorm and xx, though is able to reduce the discrepancy of gradient magnitude, are unfavorable to our model. IMTL can alleviate the task conflict considerably. We conjecture that this is because IMTL also attends the gradient direction. 
%   We qualitatively and quantitatively evaluate existing works of multi-task learning in our baseline. They are able to reduce the discrepancy of gradient magnitude and improve the subsequent performance. Throughout the paper, IMTL is adopted as the technique for inter-gradient calibration.\xd{list the average number of multi-task in table}
%   }
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{3pt}{1.0}
%   \begin{tabular}{@{}lccccc@{}}
%     \toprule
%     Method & $\gamma_{\rm task}$ &mAP(\%) & NDS &mIoU(\%) &$\Delta_{\rm MTL}$\\
%     \midrule
%     Baseline  &16.87 & 59.09 &65.03 &43.90 &-\\
%     GradNorm~\cite{chen2018gradnorm}  &12.54 & 58.33 & 64.41 & 57.19&\\
%     DWA~\cite{liu2019end} &-  &\textbf{59.29} & \textbf{65.14} & 57.72 &\\
%     IMTL~\cite{liu2021towards} &1.07  &57.07 &63.34  &\textbf{59.40} &\\
%     \bottomrule
%   \end{tabular}}
%   \label{tab:mtl_result}
% \end{table}


% \begin{table}
%   \centering
%   \caption{
%   We qualitatively and quantitatively evaluate existing works of multi-task learning in our baseline. They are able to reduce the discrepancy of gradient magnitude and improve the subsequent performance. 
%   \lsh{Note that DWA has to..}
%   % Throughout the paper, IMTL is adopted as the technique for inter-gradient calibration.
%   }\vspace{-4mm}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{5pt}{1.0}
%   \begin{tabular}{@{}lccccc@{}}
%     \toprule
%     Method & $\gamma_{\rm task}$ $^\downarrow$ &mAP(\%)$^\uparrow$ 
%     & NDS$^\uparrow$ &mIoU(\%)$^\uparrow$ &$\Delta_{\rm MTL}$(\%) $^\downarrow$\\
%     \midrule
%     Baseline  &16.87 & 59.1 &65.0 &44.0 &36.6\\
%     GradNorm~\cite{chen2018gradnorm}  &12.54 & 58.3 & 64.4 & 57.2&17.6\\
%     DWA~\cite{liu2019end} &-  &59.3 & 65.1 & 57.7 &14.1\\
%     IMTL\_G~\cite{liu2021towards} &1.13  &57.1 &63.3 &\textbf{59.4} &17.7\\
%     \midrule
%     Fuller (Ours) &1.07 &\textbf{60.5} &\textbf{65.3} &58.4 &\textbf{10.8} \\
    
%     \bottomrule
%   \end{tabular}}
%   \label{tab:mtl_result}
% \end{table}

\begin{table}
  \centering
  % \caption{We compare existing works of multi-task learning.}
  \caption{DWA needs to empirically select the initial loss weights while GradNorm uses extra learnable parameters. Considering scalability and performance, we select the IMTL\_G as the inter-gradient calibration.}
  \vspace{-0mm}
  \resizebox{1.0\columnwidth}{!}
  {\tablestyle{8pt}{1.0}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Method &mAP(\%)$\uparrow$ 
    & NDS$\uparrow$ &mIoU(\%)$\uparrow$ &$\Delta_{\rm MTL}$(\%) $\downarrow$\\
    \midrule
    Baseline  & 59.1 &65.0 &44.0 &36.6\\
    GradNorm~\cite{chen2018gradnorm}  & 58.3 & 64.4 & 57.2&17.6\\
    DWA~\cite{liu2019end}  &59.3 & 65.1 & 57.7 &14.1\\
    IMTL\_G~\cite{liu2021towards}  &57.1 &63.3 &\textbf{59.4} &17.7\\
    \midrule
    Fuller (Ours) &\textbf{60.5} &\textbf{65.3} &58.4 &\textbf{10.8} \\
    
    \bottomrule
  \end{tabular}}
  \label{tab:mtl_result}
\end{table}

==> latex/tab/task_head.tex <==
\begin{table}[!t]
  \centering
  \vspace{-1mm}
  \caption{
  Comparison between task heads.  %\gy{running experiment under 0.1 voxel size }
  }\vspace{-0mm}
\resizebox{1.0\columnwidth}{!}
{\tablestyle{10pt}{1.0}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Method  
    &mAP(\%)$\uparrow$
    & NDS$\uparrow
    $&mIoU(\%)$\uparrow$ & Params$\downarrow$\\
    \midrule
    CenterPoint\cite{yin2021center}  &58.6  & 64.8  &- & 1.6m \\
    Fuller-det (Ours) & \textbf{62.1} & \textbf{66.6} & - & \textbf{1.0m} \\
    BEVFusion\cite{liu2022bevfusion} & - & - &  \textbf{62.7} & 4.7m \\
    Fuller-seg (Ours) & - & - & 62.3 & \textbf{2.7m}\\

    \bottomrule
  \end{tabular}}\vspace{-2mm}
  \label{tab:task_head}
\end{table}

==> tab/ablation.tex <==

% \begin{table}[t]
%     \centering
%     \caption{Ablation Study.\xd{add caption, what do first lines mean}}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{1pt}{1.0}
%     \begin{tabular}{@{}cc|cccc@{}}
%     \toprule
%         % Modality Grad. & Task Grad. &mAP &NDS &mIoU\\
%         Intra-gradient & Inter-gradient &mAP(\%) &NDS &mIoU(\%) &$\Delta_{\rm MTL}$(\%)\\
%         \midrule
%         \midrule
%         \multicolumn{5}{c}{\textit{det\_loss:seg\_loss=1:1}}\\
%         \midrule
%         &  &59.09 & 65.03 & 43.97\\
%         \checkmark & &59.51 &65.36 &45.01\\
%         &\checkmark & 57.07 &63.34 &59.46\\
%         \checkmark &\checkmark &60.47  &65.34  &58.35\\
%         \midrule
%         \midrule
%         \multicolumn{5}{c}{\textit{det\_loss:seg\_loss=1:5}}\\
%         \midrule
        
%         &  &59.79 & 65.46 & 55.65 \\
%         \checkmark &  &59.83 &65.31 &56.13\\
%         &\checkmark &56.94 &63.31  &59.84\\
%         \checkmark &\checkmark & 60.13 & 65.62 & 58.24\\
%         \midrule
%         \midrule
%         \multicolumn{5}{c}{\textit{det\_loss:seg\_loss=1:10}}\\
        
%         \midrule
%         &  &59.31 & 65.00 & 57.92\\
%         \checkmark & & 60.05 & 65.41 & 57.30\\
%         &\checkmark &58.17  &64.16 & 60.05\\
%         \checkmark &\checkmark & 59.85 &65.18 &59.20\\
% \bottomrule
%     \end{tabular}}
%     \label{tab:ablation}
% \end{table}

\begin{table}[t]
    \centering
    % \caption{Ablation Study of the proposed inter-gradient and intra-gradient calibration under three different initial states.}
    \caption{Ablation Study of the proposed inter-gradient and intra-gradient calibration with three different initial states.}
    \vspace{-0mm}
    \resizebox{1.0\columnwidth}{!}
    {\tablestyle{5pt}{1.0}
    \begin{tabular}{@{}cc|cccc@{}}
    \toprule
        % Modality Grad. & Task Grad. &mAP &NDS &mIoU\\
        Intra-grad. & Inter-grad. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
        &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
        \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:1}}\\ s
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:1}}\\
        \midrule
        &  &59.1 & 65.0 & 44.0 &18.3\\
        \checkmark & &59.5 &\textbf{65.4} &45.0 &16.9\\
        &\checkmark & 57.1 &63.3 &\textbf{59.5} &8.8\\
        \checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{5.4}\\
        
        \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:5}}\\
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:5}}\\
        \midrule
        &  &59.8 & 65.5 & 55.7 &8.0\\
        \checkmark &  &59.8 &65.3 &56.1 &7.8 \\
        &\checkmark &56.9 &63.3  &\textbf{59.8} &8.7 \\
        \checkmark &\checkmark & \textbf{60.1} & \textbf{65.6} & 58.2 &\textbf{5.7}\\
        
        \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:10}}\\
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:10}}\\
        \midrule
        &  &59.3 & 65.0 & 57.9 &7.0\\
        \checkmark & & \textbf{60.1} & \textbf{65.4} & 57.3 &6.5\\
        &\checkmark &58.2  &64.2 & \textbf{60.1} &6.7\\
        \checkmark &\checkmark & 59.9 &65.2 &59.2 &\textbf{5.3}\\
\bottomrule
    \end{tabular}}
    \label{tab:ablation}\vspace{-4mm}
\end{table}

==> tab/add_new_task.tex <==
\begin{table}[t]
  \centering
  \vspace{-0mm}
  \caption{Verifying the framework with more learning tasks.}
  \vspace{-0mm}
\resizebox{1.0\columnwidth}{!}
{\tablestyle{1pt}{1.0}
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    Method  &mAP(\%)$\uparrow$ & NDS$\uparrow $&mIoU$_{\rm map}$(\%)$\uparrow$ & mIoU$_{\rm fore}$(\%)$\uparrow$ &$\Delta_{\rm MTL}$ $\downarrow$\\
    \midrule
    % Fuller-det &62.1 &66.6 &- &-\\
    % Fuller-seg &- &- &62.3 &-\\
    % LSS \\
    Upper bound &62.1 &66.6 &62.3 &63.8 &-\\
    MTL baseline &\textbf{59.9} &\textbf{65.8} & 46.9 & 58.1 &12.8\\
    Fuller &58.6 & 64.6 &\textbf{57.1} &\textbf{62.0} &\textbf{9.9}\\
    \bottomrule
  \end{tabular}}\vspace{-5mm}
  \label{tab:add_new_task}
\end{table}

==> tab/algorithm.tex <==
% \begin{algorithm}
%     \renewcommand{\algorithmicrequire}{\textbf{Input}}
% 	\renewcommand{\algorithmicensure}{\textbf{Output}}
%     \caption{Training Procedure of Fuller}
%     \label{alg:fuller}
%     \begin{algorithmic}[1]
%         % \STATE \textbf{Input} input $x_{lid}$ and $x_{img}$, ground-truth $y_{lid}$ and $y_{img}$, backbone $H$, last backbone layer $H_{last}$, fusion layer $H_{fuse}$, task heads $\phi_{lid}$ and $\phi_{img}$, learning rate $\eta$
%         \REQUIRE input $X$, ground-truth $Y$, backbone $H$, backbone's parameter $\theta^H$, task head $\phi$, task head's parameter $\theta^T$, learning rate $\eta$.
%         % \STATE \textbf{Output} backbone $H$, task head $\phi$
%         \ENSURE backbone $H$, task head $\phi$
%         \FOR {\{($x_{lid}$, $x_{img}$), {($y_{seg}$, $y_{det}$})\} in \{$X$,$Y$\}}
%         \STATE inter-gradient calibration for task conflict: \\
%         $\bigtriangledown_{H_{last}}\mathcal{L}_{\rm seg} \leftarrow \frac{\partial \mathcal{L_{\rm seg}}(\phi_{\rm seg}(H(x_{lid},x_{img})),y_{seg})}{\partial H_{last}}$ 
        
%         \STATE $\bigtriangledown_{H_{last}}\mathcal{L}_{\rm det} \leftarrow \frac{\partial \mathcal{L_{\rm det}}(\phi_{\rm det}(H(x_{lid},x_{img})),y_{det})}{\partial H_{last}}$  
        
%         \STATE $\alpha_{\rm seg}$, $\alpha_{\rm det}$ $\leftarrow$ {\rm IMTL}($\bigtriangledown_{H_{last}}\mathcal{L}_{\rm seg}$,$\bigtriangledown_{H_{last}}\mathcal{L}_{\rm det}$) 
%         \STATE $\mathcal{L}\leftarrow \alpha_{\rm seg}\cdot \mathcal{L}_{\rm seg} + \alpha_{\rm det}\cdot \mathcal{L}_{\rm det}$
%         \STATE $\theta^T \leftarrow \theta^T - \eta \cdot \frac{\partial \mathcal{L}}{\partial \theta^T}$
%         \STATE intra-gradient calibration for modality bias \\
%         $G_{lid} \leftarrow \frac{\partial \mathcal{L}}{\partial H_{fuse}}[:,:256,:,:]$
%         \STATE $G_{img} \leftarrow \frac{\partial \mathcal{L}}{\partial H_{fuse}}[:,256:,:,:]$
        
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
    \renewcommand{\algorithmicrequire}{\textbf{Input}}
	\renewcommand{\algorithmicensure}{\textbf{Output}}
    \caption{Training Procedure of Fuller}
    \label{alg:fuller}
    \begin{algorithmic}[1]
        % \STATE \textbf{Input} input $x_{lid}$ and $x_{img}$, ground-truth $y_{lid}$ and $y_{img}$, backbone $H$, last backbone layer $H_{last}$, fusion layer $H_{fuse}$, task heads $\phi_{lid}$ and $\phi_{img}$, learning rate $\eta$
        \REQUIRE 
        % input $X$, ground-truth $Y$, 
        composition function $\sigma$, 
        %shared backbone $H$, 
        modality branches' parameter $\theta^H$, 
        %task head $K$, 
        intra-gradient layer's parameter $\theta^F$,
        off-the-modality's parameter $\theta^K$, learning rate $\eta$.
        %\xd{as we have too much symbols, pls check whole paper whether each symbol is defined, where implementation details explain all parameters}
        % \STATE \textbf{Output} backbone $H$, task head $\phi$
        \ENSURE $\theta^H$, $\theta^K$
        \FOR { $t=0,1,2,...,T$}
        \STATE Inter-gradient Calibration For Task Conflict: \\ 
        
        %$\leftarrow$ {\rm IMTL}(
        %$\frac{\partial \mathcal{L}_{\rm det}}{\partial{\theta^{H}_{last}}}$,
        %$\frac{\partial \mathcal{L}_{\rm seg}}{\partial{\theta^{H}_{last}}}$)
        
        {\small $\alpha_{\rm Seg}$, $\alpha_{\rm Det}$
        $\leftarrow$ {\rm IMTL}(
        $\nabla_{\texttt{shared\_L}}\mathcal{L}_{\rm{Det}},
        \nabla_{\texttt{shared\_L}}\mathcal{L}_{\rm{Seg}}$)}

        \STATE $\mathcal{L}\leftarrow \alpha_{\rm Seg}\cdot \mathcal{L}_{\rm Seg} + \alpha_{\rm Det}\cdot \mathcal{L}_{\rm Det}$
        \STATE $\theta^K \leftarrow \theta^K - \eta \cdot \frac{\partial \mathcal{L}}{\partial \theta^K}$ \ $\triangleleft$ \ Update task heads
        % \STATE $\theta^F \leftarrow \theta^F - \eta \cdot \frac{\partial \mathcal{L}}{\partial \theta^F}$ \ $\triangleleft$ \ \ Update fusion block 
        \STATE Intra-gradient Calibration for Modality Bias: \\
        % $G^{t}_{lid} \leftarrow \frac{\partial \mathcal{L}}{\partial H_{fuse}}[:,:256,:,:]$
        
        \STATE $\nabla{\theta^{F}_{lid}},  \nabla{\theta^{F}_{img}} \leftarrow \frac{\partial \mathcal{L}}{\partial \theta^{F}_{lid}}, \frac{\partial \mathcal{L}}{\partial \theta^{F}_{img}}$
        
        % \STATE $G^{t}_{img} \leftarrow \frac{\partial \mathcal{L}}{\partial H_{fuse}}[:,256:,:,:]$
        
        \STATE $w^{t}_{lid} \leftarrow \sigma(||\nabla{{\theta^{F}_{lid}}^{t}}||,||\nabla{{\theta^{F}_{img}}^{t}}||)$\\
        $w^{t}_{img} \leftarrow \sigma(||\nabla{{\theta^{F}_{img}}^{t}}||,||\nabla{{\theta^{F}_{lid}}^{t}}||)$
        \STATE $w^{t}_{lid} \leftarrow m\cdot w^{t-1}_{lid} + (1-m)\cdot w^{t}_{lid}$ \\ %$\triangleleft$ momentum update
        $w^{t}_{img} \leftarrow m\cdot w^{t-1}_{img} + (1-m)\cdot w^{t}_{img}$ 
        \STATE $G^{t}_{lid} \leftarrow w^{t}_{lid} \cdot G^{t}_{lid}$
        ; \; $G^{t}_{img} \leftarrow w^{t}_{img} \cdot G^{t}_{img}$
        \STATE backward $G^{t}_{lid}$ and update $\theta^{H}_{lid}$ \; \; $\triangleleft$ LiDAR branch
        \STATE backward $G^{t}_{img}$ and update $\theta^{H}_{img}$ $\triangleleft$ Image branch
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

==> tab/big_table.tex <==
% \begin{table*}[h]
%     \centering
%     \caption{\textbf{Improving Baseline.} This is the baseline where det loss and seg loss are 1:1. This table is copied from Bevfusin(@mit). Please adjust it according to our settings. 
%     {\color{green}{(zj: FULLER is running)}}}
%     \begin{threeparttable}
%     \begin{tabular}{@{}l|ccccc@{}}
%     \toprule
%          \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& &\multicolumn{2}{c}{Det} &Seg \\ \cline{3-4}
%           &Modality &mAP &NDS &mIoU  \\
%           \midrule
%          PointPainting& C+L & 65.8 & 69.6 & -\\
%          MVP& C+L& 66.1 & 70.0 & -\\
%          FusionPainting & C+L &66.5 & 70.7 & - \\
%          AutoAlign & C+L & 66.6 & 71.7 & - \\
%          FUTR3D & C+L & 64.5 & 68.3 & - \\
%          TransFusion & C+L & 67.5 & 71.3 & - \\
%          BEVFusion & C+L & 68.5 & 71.4 & - \\
%          \midrule
%          PointPainting & C+L & - & - & 49.1 \\
%          MVP & C+L & - & - & 49.0 \\
%          BEVFusion & C+L & - & - & 62.7 \\
%          \midrule
%          BEVFusion$^{\dag}$\_Joint(shared BEV encoders) & C+L & - & 69.7 & 54.0\\
%          BEVFusion$^{\footnotemark[2]}$\_Joint( BEV encoders) & C+L & - & 69.9 & 58.4\\
%          Baseline$^{*}$ (upper bound) &C+L & 62.07 & 66.57 & 62.27\\
%          Baseline& C+L & 59.09 & 65.03 & 43.97\\
%          %Method 1 &\\
%          %Method 2 & \\
%          Fuller& C+L \\
%          \bottomrule
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[*] is single-task learning, served as upper bound. $^{\dag}$ balances loss weights manually.
%     \end{tablenotes}
% \end{threeparttable}
% \label{tab:baseline}
% \end{table*}


\begin{table*}[t]
    \centering
    \caption{Comparison to more methods.}
    \vspace{-0mm}
    \resizebox{2.0\columnwidth}{!}
    {\tablestyle{8pt}{1.0}
    \begin{threeparttable}

    \begin{tabular}{@{}l|cccc|ccc}
    \toprule
         % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& & & &\multicolumn{2}{c}{Det} &Seg \\ \cline{5-6}
          &Modality& VoxelSize & LiDAR &Image &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ \\
          \midrule
          \midrule
         \multicolumn{8}{c}{3D Detection}\\
          \midrule
         M$^2$BEV~\cite{xie2022m} & C & -&- & ResNeXt-101~\cite{Xie_2017_CVPR}&\cellcolor{blue!5}41.7 &\cellcolor{blue!5}47.0 & -\\
         BEVFormer~\cite{li2022bevformer} & C & -& -& ResNet101~\cite{He_2016_CVPR}&\cellcolor{blue!5}41.6 &\cellcolor{blue!5}51.7 & -\\
         PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L &0.075 &PointPillars &- &\cellcolor{blue!5}52.3 &\cellcolor{blue!5}61.3 &- \\
         CenterPoint~\cite{yin2021center} &L & 0.075&VoxelNet &- &\cellcolor{blue!5}59.6 &\cellcolor{blue!5}66.8 &- \\
         PointPainting$^{\ddag}$~\cite{vora2020pointpainting}& C+L&0.075 & PointPillars &- & \cellcolor{blue!5}65.8 &  \cellcolor{blue!5}69.6 & -\\
         MVP$^{\ddag}$~\cite{yin2021multimodal}& C+L & 0.075 &  VoxelNet & DLA-34& \cellcolor{blue!5}66.1 & \cellcolor{blue!5}70.0 & -\\
         FusionPainting~\cite{xu2021fusionpainting} & C+L & -&Cylinder3D~\cite{zhou2020cylinder3d} &HTCNet~\cite{Chen_2019_CVPR}&\cellcolor{blue!5}66.5 & \cellcolor{blue!5}70.7 & - \\
         AutoAlign~\cite{chen2022autoalign} & C+L &0.075 & CenterPoint & ResNet-50& \cellcolor{blue!5}66.6 & \cellcolor{blue!5}71.1 & - \\
         FUTR3D~\cite{chen2022futr3d} & C+L & 0.075& VoxelNet & ResNet-101& \cellcolor{blue!5}64.5 & \cellcolor{blue!5}68.3 & - \\
         TransFusion~\cite{bai2022transfusion} & C+L &0.075 & VoxelNet&DLA-34& \cellcolor{blue!5}67.5 & \cellcolor{blue!5}71.3 & - \\
         BEVFusion~\cite{liu2022bevfusion} & C+L &0.075 & VoxelNet&Swin-T &  \cellcolor{blue!5}68.5 & \cellcolor{blue!5}71.4 & - \\
         % Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.60} &\cellcolor{blue!5}\textbf{71.30}  &- \\
         % Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.07} &\cellcolor{blue!5}\textbf{66.57} &- \\
         Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.6} &\cellcolor{blue!5}\textbf{71.3}  &- \\
         Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.1} &\cellcolor{blue!5}\textbf{66.6} &- \\
         \midrule
          \midrule
         \multicolumn{8}{c}{BEV Map Segmentation}\\
          \midrule
         OFT$^{\ddag}$~\cite{roddick2018orthographic} &C  &- &- &ResNet-18 &- &- &\cellcolor{blue!5}42.1 \\
         LSS$^{\ddag}$~\cite{philion2020lift} &C  &- &- &EfficientNet-B0~\cite{tan2019efficientnet}&- &-&\cellcolor{blue!5}44.4 \\
         PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L & 0.1&- &PointPillars &- &- &\cellcolor{blue!5}43.8 \\
         CenterPoint$^{\ddag}$~\cite{yin2021center} &L &0.1  &VoxelNet &- &- &-  &\cellcolor{blue!5}48.6 \\
         PointPainting$^{\ddag}$~\cite{vora2020pointpainting} & C+L  &0.1& PointPillars & - &- &- & \cellcolor{blue!5}49.1 \\
         MVP$^{\ddag}$~\cite{yin2021multimodal} & C+L &0.1 & VoxelNet & DLA-34\cite{yu2018deep}  &- &- & \cellcolor{blue!5}49.0 \\
         BEVFusion~\cite{liu2022bevfusion} & C+L  &0.1 & VoxelNet&Swin-T & -&- & \cellcolor{blue!5}62.7 \\
         % Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.27} \\
         Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.3} \\
         \midrule
          \midrule
         \multicolumn{8}{c}{3D Detection + BEV Map Segmentation}\\
          \midrule
         BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (share) & C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}- & \cellcolor{blue!5}69.7 & \cellcolor{blue!5}54.0\\
         BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (sep) & C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}- & \cellcolor{blue!5}69.9 & \cellcolor{blue!5}58.4\\
         % Baseline$^{*}$ (upper bound) &C+L &D+S & 62.07 & 66.57 & 62.27\\
         % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.09} & \cellcolor{blue!5}\textbf{65.03} & \cellcolor{blue!5}\textbf{43.97}\\
         % Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.47} &\cellcolor{blue!5}\textbf{65.34}  &\cellcolor{blue!5}\textbf{58.35}\\
         % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.1} & \cellcolor{blue!5}\textbf{65.0} & \cellcolor{blue!5}\textbf{44.0}\\
         Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}59.1 & \cellcolor{blue!5}65.0 & \cellcolor{blue!5}44.0\\
         Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.5} &\cellcolor{blue!5}\textbf{65.3}  &\cellcolor{blue!5}\textbf{58.4}\\
         \bottomrule
    \end{tabular}
    % \begin{tablenotes}
    %     \footnotesize
    %     \item[$\dag$] means the multi-task result in BEVFusion\cite{liu2022bevfusion}. $^{\ddag}$ means re-implementation result in BEVFusion\cite{liu2022bevfusion}. `share' means multi-task heads share one BEV encoder to process the fused multimodal feature. `sep' means task heads have separate encoders.
    % \end{tablenotes}
\end{threeparttable}}
\vspace{-3mm}
\label{tab:more_comparison}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \caption{Comparison with benchmark. The upper two sub-tables are single task results while the bottom one is multi-task result.‘L’ and ‘C’ represent LiDAR and Camera, respectively. We treat single task result as our upper bound because multi-task will generally decrease the performance. Baseline means Fuller is naively trained where detection loss and segmentation loss are set to 1:1. `-' means inapplicable.
%     %\xd{can remove some old methods into appendix}
%     }\vspace{-3mm}
%     \resizebox{2.0\columnwidth}{!}
%     {\tablestyle{5pt}{1.0}
%     \begin{threeparttable}

%     \begin{tabular}{@{}l|cccc|cccc}
%     \toprule
%          % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& & & &\multicolumn{2}{c}{Det} &Seg \\ \cline{5-6}
%           &Modality& VoxelSize & LiDAR &Image &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ &$\Delta_{\rm MTL}$(\%)$\downarrow$\\
%           \midrule
%           \midrule
%          \multicolumn{9}{c}{3D Detection}\\
%           \midrule
%         %  M$^2$BEV~\cite{xie2022m} & C & -&- & ResNeXt-101~\cite{Xie_2017_CVPR}&\cellcolor{blue!5}41.7 &\cellcolor{blue!5}47.0 & -\\
%          BEVFormer~\cite{li2022bevformer} & C &- &- & ResNet101~\cite{He_2016_CVPR}& 41.6 & 51.7 & - &-\\
%         %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L &0.075 &PointPillars &- &\cellcolor{blue!5}52.3 &\cellcolor{blue!5}61.3 &- \\
%          CenterPoint~\cite{yin2021center} &L & 0.075&VoxelNet &- & 59.6 & 66.8 &- &-\\
%         %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting}& C+L&0.075 & PointPillars &- & \cellcolor{blue!5}65.8 &  \cellcolor{blue!5}69.6 & -\\
%          MVP$^{\ddag}$~\cite{yin2021multimodal}& C+L & 0.075 &  VoxelNet & DLA-34&  66.1 &  70.0 &- &-\\
%         %  FusionPainting~\cite{xu2021fusionpainting} & C+L & -&Cylinder3D~\cite{zhou2020cylinder3d} &HTCNet~\cite{Chen_2019_CVPR}&\cellcolor{blue!5}66.5 & \cellcolor{blue!5}70.7 & - \\
%         %  AutoAlign~\cite{chen2022autoalign} & C+L &0.075 & CenterPoint & ResNet-50& \cellcolor{blue!5}66.6 & \cellcolor{blue!5}71.1 & - \\
%          % FUTR3D~\cite{chen2022futr3d} & C+L & 0.075& VoxelNet & ResNet-101& \cellcolor{blue!5}64.5 & \cellcolor{blue!5}68.3 & - \\
%          TransFusion~\cite{bai2022transfusion} & C+L &0.075 & VoxelNet&DLA-34&  67.5 &  71.3 &- &-\\
%          BEVFusion~\cite{liu2022bevfusion} & C+L &0.075 & VoxelNet&Swin-T &   68.5 &  71.4 & - &-\\
%          % Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.60} &\cellcolor{blue!5}\textbf{71.30}  &- \\
%          % Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.07} &\cellcolor{blue!5}\textbf{66.57} &- \\
%          Fuller-det &C+L  &0.075 & VoxelNet&Swin-T &  67.6 & 71.3  &- &-\\
%          Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T &  \textbf{62.1} & \textbf{66.6} &- &-\\
%          \midrule
%           \midrule
%          \multicolumn{9}{c}{BEV Map Segmentation}\\
%           \midrule
%         %  OFT$^{\ddag}$~\cite{roddick2018orthographic} &C  &- &- &ResNet-18 &- &- &\cellcolor{blue!5}42.1 \\
%          LSS$^{\ddag}$~\cite{philion2020lift} &C  &- &- &EfficientNet-B0&- &-& 44.4 &-\\
%         %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L & 0.1&- &PointPillars &- &- &\cellcolor{blue!5}43.8 \\
%          CenterPoint$^{\ddag}$~\cite{yin2021center} &L &0.1  &VoxelNet &- &- &-  & 48.6 &-\\
%         %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting} & C+L  &0.1& PointPillars & - &- &- & \cellcolor{blue!5}49.1 \\
%          % MVP$^{\ddag}$~\cite{yin2021multimodal} & C+L &0.1 & VoxelNet & DLA-34\cite{yu2018deep}  &- &- & \cellcolor{blue!5}49.0 \\
%          BEVFusion~\cite{liu2022bevfusion} & C+L  &0.1 & VoxelNet&Swin-T & -&- &  62.7 &-\\
%          % Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.27} \\
%          Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - & \textbf{62.3} &-\\
%          \midrule
%           \midrule
%          \multicolumn{9}{c}{3D Detection + BEV Map Segmentation}\\
%           \midrule
%          BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (share) & C+L  &0.1 & VoxelNet&Swin-T & - &  69.7 &  54.0 &-\\
%          BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (sep) & C+L  &0.1 &VoxelNet&Swin-T &  - &  69.9 &  58.4 &-\\
%          % Baseline$^{*}$ (upper bound) &C+L &D+S & 62.07 & 66.57 & 62.27\\
%          % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.09} & \cellcolor{blue!5}\textbf{65.03} & \cellcolor{blue!5}\textbf{43.97}\\
%          % Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.47} &\cellcolor{blue!5}\textbf{65.34}  &\cellcolor{blue!5}\textbf{58.35}\\
%          Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T&  {59.1} &  {65.0} &  {44.0} & {33.6}\\
%          Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T & \textbf{60.5} & \textbf{65.3}  & \textbf{58.4} & \textbf{10.8}\\
%          \bottomrule
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[$\dag$] means the multi-task result in BEVFusion\cite{liu2022bevfusion}. $^{\ddag}$ means re-implementation result in BEVFusion\cite{liu2022bevfusion}. `share' means multi-task heads share one BEV encoder to process the fused multimodal feature. `sep' means task heads have separate encoders.
%     \end{tablenotes}
% \end{threeparttable}}
% \vspace{-3mm}
% \label{tab:baseline}
% \end{table*}

==> tab/diff_setting.tex <==
% \begin{table}[t]
%     \centering
%     \caption{\textbf{Sensitivity Analysis.}\xd{bold all best numbers in all tables} From a retrospective view, we find that increasing the weight of segmentation loss is beneficial to gradient balancing. Rather than 1:1, we increase the initial weight of segmentation loss to investigate to what extent the proposed model can still improve the baseline model. }
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{5pt}{1.0}
%     \begin{tabular}{@{}l|c|ccccc@{}}
%     \toprule
%          % & &\multicolumn{2}{c}{Det} &Map Seg. \\ \cline{3-4}
%          &weight ratio  &mAP(\%) &NDS &mIoU(\%) &$\Delta_{\rm MTL}$ \\
%          \midrule
%          Baseline&\multirow{2}{*}{1:1} & 59.09 & 65.03 &43.97 &-\\
%          Fuller& &60.47  &65.34  &58.35 &\\
%          \midrule
%          Baseline&\multirow{2}{*}{1:5} &59.79 & 65.46 & 55.65 &-\\
%          Fuller & & 60.13 & 65.62 & 58.24\\
%          \midrule
%          Baseline&\multirow{2}{*}{1:10} &59.31 & 65.00 & 57.92 &-\\
%          Fuller & &59.85 & 65.18 & 59.20\\
%          \bottomrule
%     \end{tabular}}
%     \label{tab:sensitiviy}
% \end{table}

% \begin{table}[t]
%     \centering
%     \caption{Sensitivity analysis on initial loss weights. 
%     % From a retrospective view, we find that increasing the weight of segmentation loss is beneficial to gradient balancing.
%     Rather than 1:1, we increase the initial weight of segmentation loss to investigate to what extent the proposed model can still improve the baseline model. }\vspace{0mm}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{5pt}{1.0}
%     \begin{tabular}{@{}l|c|ccccc@{}}
%     \toprule
%          % & &\multicolumn{2}{c}{Det} &Map Seg. \\ \cline{3-4}
%          &weight ratio  &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
%          &$\Delta_{\rm MTL}$(\%) $\downarrow$\\
%          \midrule
%          Baseline&\multirow{2}{*}{1:1} & 59.1 & 65.0 &44.0 &36.6\\
%          Fuller& &\textbf{60.5}  &\textbf{65.3}  &\textbf{58.4} &\textbf{10.8}\\
%          \midrule
%          Baseline&\multirow{2}{*}{1:5} &59.8 & 65.5 & 55.7 &16.0\\
%          Fuller & & \textbf{60.1} & \textbf{65.6} & \textbf{58.2} &\textbf{11.3}\\
%          \midrule
%          Baseline&\multirow{2}{*}{1:10} &59.3 & 65.0 & 57.9 &14.0\\
%          Fuller & &\textbf{59.9} & \textbf{65.2} & \textbf{59.2} &\textbf{10.6}\\
%          \bottomrule
%     \end{tabular}}
%     \label{tab:sensitiviy}\vspace{0mm}
% \end{table}


\begin{table}[t]
    \centering
    % \caption{Ablation Study of the proposed inter-gradient and intra-gradient calibration under three different initial states.}
    % \caption{Sensitivity analysis and ablation study of the proposed inter-gradient and intra-gradient calibration with three different initial states.}
    \caption{Sensitivity analysis and ablation study of the proposed gradient calibration with different initial loss weights.}
    \vspace{-0mm}
    \resizebox{1.0\columnwidth}{!}
    {\tablestyle{8pt}{1.0}
    \begin{tabular}{@{}cc|cccc@{}}
    \toprule
        % Modality Grad. & Task Grad. &mAP &NDS &mIoU\\
        Intra. & Inter. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
        &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
        \midrule
        % \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:1}}\\ s
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:1}}\\
        \midrule
        &  &59.1 & 65.0 & 44.0 &18.3\\
        \checkmark & &59.5 &\textbf{65.4} &45.0 &16.9\\
        &\checkmark & 57.1 &63.3 &\textbf{59.5} &8.8\\
        \checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{5.4}\\
        
        % \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:5}}\\
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:5}}\\
        \midrule
        &  &59.8 & 65.5 & 55.7 &8.0\\
        \checkmark &  &59.8 &65.3 &56.1 &7.8 \\
        &\checkmark &56.9 &63.3  &\textbf{59.8} &8.7 \\
        \checkmark &\checkmark & \textbf{60.1} & \textbf{65.6} & 58.2 &\textbf{5.7}\\
        
        % \midrule
        \midrule
        % \multicolumn{6}{c}{\textit{det\_loss:seg\_loss=1:10}}\\
        \multicolumn{6}{c}{\textit{det\_weight:seg\_weight=1:10}}\\
        \midrule
        &  &59.3 & 65.0 & 57.9 &7.0\\
        \checkmark & & \textbf{60.1} & \textbf{65.4} & 57.3 &6.5\\
        &\checkmark &58.2  &64.2 & \textbf{60.1} &6.7\\
        \checkmark &\checkmark & 59.9 &65.2 &59.2 &\textbf{5.3}\\
\bottomrule
    \end{tabular}}
    \label{tab:ablation}\vspace{-4mm}
\end{table}

==> tab/disjoint.tex <==
% \begin{table}[]
%     \centering
%     \caption{Results on different dataset settings. The Full setting has the complete annotations and thus is the upper bound.\lsh{plz change the number to xx.x}}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{3pt}{1.1}
%     \begin{tabular}{@{}l|l|cccc@{}}
%     \toprule
%         Setting &Method &mAP(\%) &NDS &mIoU(\%) &$\Delta_{\rm MTL}$(\%)\\
%         \hline
%         \multirow{2}{*}{Full}  &Baseline &59.09 &65.03 &43.97\\      
%          & Fuller &60.47  &65.34  &58.35\\
%          \hline
%         \multirow{2}{*}{Disjoint-balance}  &Baseline & 58.71 & 64.16& 41.53\\      
%          & Fuller \\
%          \hline
%         \multirow{2}{*}{Disjoint-normal}  &Baseline &59.11 & 64.67 & 43.14\\      
%          & Fuller &58.94 &64.92 &55.03\\
         
%          \bottomrule
%     \end{tabular}}
%     \label{tab:disjoint}
% \end{table}

% \begin{table}[]
%     \centering
%     \caption{Results on different dataset settings. The Full setting has the complete annotations and thus is the upper bound.}\vspace{-0mm}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{3pt}{1.1}
%     \begin{tabular}{@{}l|l|cccc@{}}
%     \toprule
%         Setting &Method &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
%         &$\Delta_{\rm MTL}$(\%)$\downarrow$\\
%         \hline
%         \multirow{2}{*}{Full}  &Baseline &59.1 &65.0 &44.0 &33.6\\      
%          & Fuller &\textbf{60.5}  &\textbf{65.3}  &\textbf{58.4} &\textbf{10.8}\\
%          \hline
%         \multirow{2}{*}{Disjoint-balance}  &Baseline & \textbf{58.7} & \textbf{64.2}& 41.5 &42.5 \\      
%          & Fuller &58.4 &63.6 &\textbf{56.7} &\textbf{19.5}\\
%          \hline
%         \multirow{2}{*}{Disjoint-normal}  &Baseline &\textbf{59.1} & 64.7 & 43.1 &38.5\\      
%          & Fuller &58.9 &\textbf{64.9} &\textbf{55.0} &\textbf{19.4}\\
         
%          \bottomrule
%     \end{tabular}}
%     \label{tab:disjoint}\vspace{-1mm}
% \end{table}

% \begin{table}[t]
%     \centering
%     % \caption{Sensitivity analysis and ablation study of the proposed inter-gradient and intra-gradient calibration under different dataset distribution.}
%     \caption{Sensitivity analysis and ablation study of the proposed gradient calibration under different dataset distribution.}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{4pt}{1.0}
%     \begin{tabular}{@{}ccc|cccc@{}}
%     \toprule
%         Setting &Intra. & Inter. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
%         &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
%         \midrule
%         \multirow{4}{*}{\rotatebox{90}{Full}} & & &59.1 & 65.0 & 44.0 &36.6\\
%         &\checkmark & &59.5 &\textbf{65.4} &45.0 &33.8\\
%         & &\checkmark & 57.1 &63.3 &\textbf{59.5} &17.5\\
%         &\checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{10.8}\\
%         \midrule
%         \multirow{4}{*}{\rotatebox{90}{Dj.-bala.}} & & &\textbf{58.7} & 64.2 & 41.5 &42.5\\
%         &\checkmark &  &58.3 &\textbf{65.0} &42.4 &40.5 \\
%         & &\checkmark &57.4 &62.7  &\textbf{57.3} &21.5 \\
%         & \checkmark &\checkmark & 58.4 & 63.6 & 56.7 &\textbf{19.5}\\
%         \midrule
%         \multirow{4}{*}{\rotatebox{90}{Dj.-norm.}}& &&59.1 & 64.7 & 43.1 &38.5\\
%         &\checkmark & &\textbf{59.3} &\textbf{65.3}  &44.0  &35.8\\
%         & &\checkmark &57.4  &62.9 & 53.8 &26.8\\
%         & \checkmark &\checkmark & 58.9 &64.9 &\textbf{55.0} &\textbf{19.4}\\
% \bottomrule
%     \end{tabular}}
%     \label{tab:disjoint_ablation}
% \end{table}

\begin{table}[!t]
    \centering
    % \caption{Sensitivity analysis and ablation study of the proposed inter-gradient and intra-gradient calibration under different dataset distribution.}
    \caption{Sensitivity analysis and ablation study of the proposed gradient calibration under different dataset distribution.}
    \resizebox{1.0\columnwidth}{!}
    {\tablestyle{8pt}{1.0}
    \begin{tabular}{@{}cc|cccc@{}}
    \toprule
        Intra. & Inter. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
        &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
        \midrule
        \multicolumn{6}{c}{\textit{Full}}\\
        \midrule
         & &59.1 & 65.0 & 44.0 &18.3\\
        \checkmark & &59.5 &\textbf{65.4} &45.0 &16.9\\
        &\checkmark & 57.1 &63.3 &\textbf{59.5} &8.8\\
        \checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{5.4}\\
        \midrule
        \multicolumn{6}{c}{\textit{Disjoint-balance}}\\
        \midrule
         & &\textbf{58.7} & 64.2 & 41.5 &21.3\\
        \checkmark &  &58.3 &\textbf{65.0} &42.4 &20.5 \\
        &\checkmark &57.4 &62.7  &\textbf{57.3} &10.8 \\
        \checkmark &\checkmark & 58.4 & 63.6 & 56.7 &\textbf{9.8}\\
        \midrule
        \multicolumn{6}{c}{\textit{Disjoint-normal}}\\
        \midrule
        &&59.1 & 64.7 & 43.1 &19.3\\
        \checkmark & &\textbf{59.3} &\textbf{65.3}  &44.0  &17.9\\
        &\checkmark &57.4  &62.9 & 53.8 &13.4\\
        \checkmark &\checkmark & 58.9 &64.9 &\textbf{55.0} &\textbf{9.7}\\
\bottomrule
    \end{tabular}}
    \label{tab:disjoint_ablation}
    \vspace{-4mm}
\end{table}

==> tab/disjoint_ablation.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Verifying the proposed inter-gradient and intra-gradient calibration under disjoint dataset.}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{5pt}{0.5}
%     \begin{tabular}{@{}ccc|cccc@{}}
%     \toprule
%         Setting &Intra. & Inter. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
%         &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
%         \midrule
%         \multirow{2}{*}{\rotatebox{90}{Full}} & & &59.1 & 65.0 & 44.0 &36.6\\
%         &\checkmark & &59.5 &\textbf{65.4} &45.0 &33.8\\
%         & &\checkmark & 57.1 &63.3 &\textbf{59.5} &17.5\\
%         &\checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{10.8}\\
%         \midrule
%         \multirow{2}{*}{\rotatebox{90}{Dj.-bl.}} & & &\textbf{58.7} & 64.2 & 41.5 &42.5\\
%         &\checkmark &  &58.3 &\textbf{65.0} &42.4 &40.5 \\
%         & &\checkmark &57.4 &62.7  &\textbf{57.3} &21.5 \\
%         & \checkmark &\checkmark & 58.4 & 63.6 & 56.7 &\textbf{19.5}\\
%         \midrule
%         \multirow{2}{*}{\rotatebox{90}{Dj.-nm.}}& &&59.1 & 64.7 & 43.1 &38.5\\
%         &\checkmark & &\textbf{59.3} &\textbf{65.3}  &44.0  &35.8\\
%         & &\checkmark &57.4  &62.9 & 53.8 &26.8\\
%         & \checkmark &\checkmark & 58.9 &64.9 &\textbf{55.0} &\textbf{19.4}\\
% \bottomrule
%     \end{tabular}}
%     \label{tab:disjoint_ablation}
% \end{table}

\begin{table}[t]
    \centering
    \caption{Verifying the proposed inter-gradient and intra-gradient calibration under disjoint dataset.}
    \resizebox{1.0\columnwidth}{!}
    {\tablestyle{5pt}{0.9}
    \begin{tabular}{@{}ccc|cccc@{}}
    \toprule
        Setting &Intra. & Inter. &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ 
        &{ $\Delta_{\rm MTL}$}(\%)$\downarrow$\\
        \midrule
        % \multirow{2}{*}{\rotatebox{90}{Full}} & & &59.1 & 65.0 & 44.0 &36.6\\
        % &\checkmark & &59.5 &\textbf{65.4} &45.0 &33.8\\
        % & &\checkmark & 57.1 &63.3 &\textbf{59.5} &17.5\\
        % &\checkmark &\checkmark &\textbf{60.5}  &65.3  &58.4 &\textbf{10.8}\\
        % \midrule
        
        \multirow{2}{*}{\rotatebox{90}{Dj.-bala.}} 
         % \multirow{4}{*}{balance} 
        & & &\textbf{58.7} & 64.2 & 41.5 &42.5\\
        &\checkmark &  &58.3 &\textbf{65.0} &42.4 &40.5 \\
        & &\checkmark &57.4 &62.7  &\textbf{57.3} &21.5 \\
        & \checkmark &\checkmark & 58.4 & 63.6 & 56.7 &\textbf{19.5}\\
        \midrule
        \multirow{2}{*}{\rotatebox{90}{Dj.-norm.}}
        % \multirow{4}{*}{normal}
        & &&59.1 & 64.7 & 43.1 &38.5\\
        &\checkmark & &\textbf{59.3} &\textbf{65.3}  &44.0  &35.8\\
        & &\checkmark &57.4  &62.9 & 53.8 &26.8\\
        & \checkmark &\checkmark & 58.9 &64.9 &\textbf{55.0} &\textbf{19.4}\\
\bottomrule
    \end{tabular}}
    \label{tab:disjoint_ablation}
\end{table}

==> tab/efficiency.tex <==
\begin{table}[t]
  % \vspace{-2mm}
    \centering
  \caption{Memory cost and inference speed. All the speeds are evaluated on an Tesla V100 GPU.}
  % \caption{ {\footnotesize Efficiency comparison. Evaluations are conducted with a V100 GPU (32GB) and a Xeon CPU (96 cores).} }
\resizebox{1.0\columnwidth}{!}
{
\tablestyle{22pt}{1.0}
  \begin{tabular}{@{}cccc@{}}
    \toprule
    & Memory$\downarrow$ & Parameter$\downarrow$ & FPS$\uparrow$ 
     \\
     \midrule
    STL & 6144MB & 81.97M & 1.20  \\
    FULLER & 3103MB &  44.12M & 2.30 \\
    \bottomrule
  \end{tabular}}\vspace{-3mm}
  \label{tab:efficiency}
\end{table}

==> tab/improve_baseline.tex <==
% \begin{table*}[h]
%     \centering
%     \caption{\textbf{Improving Baseline.} This is the baseline where det loss and seg loss are 1:1. This table is copied from Bevfusin(@mit). Please adjust it according to our settings. 
%     {\color{green}{(zj: FULLER is running)}}}
%     \begin{threeparttable}
%     \begin{tabular}{@{}l|ccccc@{}}
%     \toprule
%          \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& &\multicolumn{2}{c}{Det} &Seg \\ \cline{3-4}
%           &Modality &mAP &NDS &mIoU  \\
%           \midrule
%          PointPainting& C+L & 65.8 & 69.6 & -\\
%          MVP& C+L& 66.1 & 70.0 & -\\
%          FusionPainting & C+L &66.5 & 70.7 & - \\
%          AutoAlign & C+L & 66.6 & 71.7 & - \\
%          FUTR3D & C+L & 64.5 & 68.3 & - \\
%          TransFusion & C+L & 67.5 & 71.3 & - \\
%          BEVFusion & C+L & 68.5 & 71.4 & - \\
%          \midrule
%          PointPainting & C+L & - & - & 49.1 \\
%          MVP & C+L & - & - & 49.0 \\
%          BEVFusion & C+L & - & - & 62.7 \\
%          \midrule
%          BEVFusion$^{\dag}$\_Joint(shared BEV encoders) & C+L & - & 69.7 & 54.0\\
%          BEVFusion$^{\footnotemark[2]}$\_Joint( BEV encoders) & C+L & - & 69.9 & 58.4\\
%          Baseline$^{*}$ (upper bound) &C+L & 62.07 & 66.57 & 62.27\\
%          Baseline& C+L & 59.09 & 65.03 & 43.97\\
%          %Method 1 &\\
%          %Method 2 & \\
%          Fuller& C+L \\
%          \bottomrule
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[*] is single-task learning, served as upper bound. $^{\dag}$ balances loss weights manually.
%     \end{tablenotes}
% \end{threeparttable}
% \label{tab:baseline}
% \end{table*}


\begin{table*}[t]
    \centering
    \caption{Comparison with benchmark. The upper two sub-tables are single task results while the bottom one is multi-task result.‘L’ and ‘C’ represent LiDAR and Camera, respectively. We treat single task result as our upper bound because multi-task will generally decrease the performance. Baseline means Fuller is naively trained where detection loss and segmentation loss are set to 1:1. `-' means inapplicable.
    %\xd{can remove some old methods into appendix}
    }\vspace{-0mm}
    \resizebox{2.0\columnwidth}{!}
    {\tablestyle{8pt}{1.0}
    \begin{threeparttable}

    \begin{tabular}{@{}l|cccc|ccc}
    \toprule
         % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& & & &\multicolumn{2}{c}{Det} &Seg \\ \cline{5-6}
          &Modality& VoxelSize & LiDAR &Image &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ \\
          \midrule
          \midrule
         \multicolumn{8}{c}{3D Detection}\\
          \midrule
        %  M$^2$BEV~\cite{xie2022m} & C & -&- & ResNeXt-101~\cite{Xie_2017_CVPR}&\cellcolor{blue!5}41.7 &\cellcolor{blue!5}47.0 & -\\
         BEVFormer~\cite{li2022bevformer} & C & -& -& ResNet101~\cite{He_2016_CVPR}&\cellcolor{blue!5}41.6 &\cellcolor{blue!5}51.7 & -\\
        %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L &0.075 &PointPillars &- &\cellcolor{blue!5}52.3 &\cellcolor{blue!5}61.3 &- \\
         CenterPoint~\cite{yin2021center} &L & 0.075&VoxelNet &- &\cellcolor{blue!5}59.6 &\cellcolor{blue!5}66.8 &- \\
        %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting}& C+L&0.075 & PointPillars &- & \cellcolor{blue!5}65.8 &  \cellcolor{blue!5}69.6 & -\\
         MVP$^{\ddag}$~\cite{yin2021multimodal}& C+L & 0.075 &  VoxelNet & DLA-34& \cellcolor{blue!5}66.1 & \cellcolor{blue!5}70.0 & -\\
        %  FusionPainting~\cite{xu2021fusionpainting} & C+L & -&Cylinder3D~\cite{zhou2020cylinder3d} &HTCNet~\cite{Chen_2019_CVPR}&\cellcolor{blue!5}66.5 & \cellcolor{blue!5}70.7 & - \\
        %  AutoAlign~\cite{chen2022autoalign} & C+L &0.075 & CenterPoint & ResNet-50& \cellcolor{blue!5}66.6 & \cellcolor{blue!5}71.1 & - \\
         % FUTR3D~\cite{chen2022futr3d} & C+L & 0.075& VoxelNet & ResNet-101& \cellcolor{blue!5}64.5 & \cellcolor{blue!5}68.3 & - \\
         TransFusion~\cite{bai2022transfusion} & C+L &0.075 & VoxelNet&DLA-34& \cellcolor{blue!5}67.5 & \cellcolor{blue!5}71.3 & - \\
         BEVFusion~\cite{liu2022bevfusion} & C+L &0.075 & VoxelNet&Swin-T &  \cellcolor{blue!5}68.5 & \cellcolor{blue!5}71.4 & - \\
         % Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.60} &\cellcolor{blue!5}\textbf{71.30}  &- \\
         % Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.07} &\cellcolor{blue!5}\textbf{66.57} &- \\
         Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.6} &\cellcolor{blue!5}\textbf{71.3}  &- \\
         Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.1} &\cellcolor{blue!5}\textbf{66.6} &- \\
         \midrule
          \midrule
         \multicolumn{8}{c}{BEV Map Segmentation}\\
          \midrule
        %  OFT$^{\ddag}$~\cite{roddick2018orthographic} &C  &- &- &ResNet-18 &- &- &\cellcolor{blue!5}42.1 \\
         LSS$^{\ddag}$~\cite{philion2020lift} &C  &- &- &EfficientNet-B0&- &-&\cellcolor{blue!5}44.4 \\
        %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L & 0.1&- &PointPillars &- &- &\cellcolor{blue!5}43.8 \\
         CenterPoint$^{\ddag}$~\cite{yin2021center} &L &0.1  &VoxelNet &- &- &-  &\cellcolor{blue!5}48.6 \\
        %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting} & C+L  &0.1& PointPillars & - &- &- & \cellcolor{blue!5}49.1 \\
         % MVP$^{\ddag}$~\cite{yin2021multimodal} & C+L &0.1 & VoxelNet & DLA-34\cite{yu2018deep}  &- &- & \cellcolor{blue!5}49.0 \\
         BEVFusion~\cite{liu2022bevfusion} & C+L  &0.1 & VoxelNet&Swin-T & -&- & \cellcolor{blue!5}62.7 \\
         % Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.27} \\
         Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.3} \\
         \midrule
          \midrule
         \multicolumn{8}{c}{3D Detection + BEV Map Segmentation}\\
          \midrule
         BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (share) & C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}- & \cellcolor{blue!5}69.7 & \cellcolor{blue!5}54.0\\
         BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (sep) & C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}- & \cellcolor{blue!5}69.9 & \cellcolor{blue!5}58.4\\
         % Baseline$^{*}$ (upper bound) &C+L &D+S & 62.07 & 66.57 & 62.27\\
         % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.09} & \cellcolor{blue!5}\textbf{65.03} & \cellcolor{blue!5}\textbf{43.97}\\
         % Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.47} &\cellcolor{blue!5}\textbf{65.34}  &\cellcolor{blue!5}\textbf{58.35}\\
         % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.1} & \cellcolor{blue!5}\textbf{65.0} & \cellcolor{blue!5}\textbf{44.0}\\
         Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}59.1 & \cellcolor{blue!5}65.0 & \cellcolor{blue!5}44.0\\
         Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.5} &\cellcolor{blue!5}\textbf{65.3}  &\cellcolor{blue!5}\textbf{58.4}\\
         \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
        \item[$\dag$] means the multi-task result in BEVFusion\cite{liu2022bevfusion}. $^{\ddag}$ means re-implementation result in BEVFusion\cite{liu2022bevfusion}. `share' means multi-task heads share one BEV encoder to process the fused multimodal feature. `sep' means task heads have separate encoders.
    \end{tablenotes}
\end{threeparttable}}
\vspace{-3mm}
\label{tab:baseline}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \caption{Comparison with benchmark. The upper two sub-tables are single task results while the bottom one is multi-task result.‘L’ and ‘C’ represent LiDAR and Camera, respectively. We treat single task result as our upper bound because multi-task will generally decrease the performance. Baseline means Fuller is naively trained where detection loss and segmentation loss are set to 1:1. `-' means inapplicable.
%     %\xd{can remove some old methods into appendix}
%     }\vspace{-3mm}
%     \resizebox{2.0\columnwidth}{!}
%     {\tablestyle{5pt}{1.0}
%     \begin{threeparttable}

%     \begin{tabular}{@{}l|cccc|cccc}
%     \toprule
%          % \multicolumn{1}{c|}{\multirow{2}{*}{Method}}& & & &\multicolumn{2}{c}{Det} &Seg \\ \cline{5-6}
%           &Modality& VoxelSize & LiDAR &Image &mAP(\%)$\uparrow$ &NDS$\uparrow$ &mIoU(\%)$\uparrow$ &$\Delta_{\rm MTL}$(\%)$\downarrow$\\
%           \midrule
%           \midrule
%          \multicolumn{9}{c}{3D Detection}\\
%           \midrule
%         %  M$^2$BEV~\cite{xie2022m} & C & -&- & ResNeXt-101~\cite{Xie_2017_CVPR}&\cellcolor{blue!5}41.7 &\cellcolor{blue!5}47.0 & -\\
%          BEVFormer~\cite{li2022bevformer} & C &- &- & ResNet101~\cite{He_2016_CVPR}& 41.6 & 51.7 & - &-\\
%         %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L &0.075 &PointPillars &- &\cellcolor{blue!5}52.3 &\cellcolor{blue!5}61.3 &- \\
%          CenterPoint~\cite{yin2021center} &L & 0.075&VoxelNet &- & 59.6 & 66.8 &- &-\\
%         %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting}& C+L&0.075 & PointPillars &- & \cellcolor{blue!5}65.8 &  \cellcolor{blue!5}69.6 & -\\
%          MVP$^{\ddag}$~\cite{yin2021multimodal}& C+L & 0.075 &  VoxelNet & DLA-34&  66.1 &  70.0 &- &-\\
%         %  FusionPainting~\cite{xu2021fusionpainting} & C+L & -&Cylinder3D~\cite{zhou2020cylinder3d} &HTCNet~\cite{Chen_2019_CVPR}&\cellcolor{blue!5}66.5 & \cellcolor{blue!5}70.7 & - \\
%         %  AutoAlign~\cite{chen2022autoalign} & C+L &0.075 & CenterPoint & ResNet-50& \cellcolor{blue!5}66.6 & \cellcolor{blue!5}71.1 & - \\
%          % FUTR3D~\cite{chen2022futr3d} & C+L & 0.075& VoxelNet & ResNet-101& \cellcolor{blue!5}64.5 & \cellcolor{blue!5}68.3 & - \\
%          TransFusion~\cite{bai2022transfusion} & C+L &0.075 & VoxelNet&DLA-34&  67.5 &  71.3 &- &-\\
%          BEVFusion~\cite{liu2022bevfusion} & C+L &0.075 & VoxelNet&Swin-T &   68.5 &  71.4 & - &-\\
%          % Fuller-det &C+L  &0.075 & VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{67.60} &\cellcolor{blue!5}\textbf{71.30}  &- \\
%          % Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T & \cellcolor{blue!5}\textbf{62.07} &\cellcolor{blue!5}\textbf{66.57} &- \\
%          Fuller-det &C+L  &0.075 & VoxelNet&Swin-T &  67.6 & 71.3  &- &-\\
%          Fuller-det (upper bound) &C+L  &0.1 &VoxelNet&Swin-T &  \textbf{62.1} & \textbf{66.6} &- &-\\
%          \midrule
%           \midrule
%          \multicolumn{9}{c}{BEV Map Segmentation}\\
%           \midrule
%         %  OFT$^{\ddag}$~\cite{roddick2018orthographic} &C  &- &- &ResNet-18 &- &- &\cellcolor{blue!5}42.1 \\
%          LSS$^{\ddag}$~\cite{philion2020lift} &C  &- &- &EfficientNet-B0&- &-& 44.4 &-\\
%         %  PointPillars$^{\ddag}$~\cite{lang2019pointpillars} &L & 0.1&- &PointPillars &- &- &\cellcolor{blue!5}43.8 \\
%          CenterPoint$^{\ddag}$~\cite{yin2021center} &L &0.1  &VoxelNet &- &- &-  & 48.6 &-\\
%         %  PointPainting$^{\ddag}$~\cite{vora2020pointpainting} & C+L  &0.1& PointPillars & - &- &- & \cellcolor{blue!5}49.1 \\
%          % MVP$^{\ddag}$~\cite{yin2021multimodal} & C+L &0.1 & VoxelNet & DLA-34\cite{yu2018deep}  &- &- & \cellcolor{blue!5}49.0 \\
%          BEVFusion~\cite{liu2022bevfusion} & C+L  &0.1 & VoxelNet&Swin-T & -&- &  62.7 &-\\
%          % Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - &\cellcolor{blue!5}\textbf{62.27} \\
%          Fuller-seg(upper bound) &C+L  &0.1 &VoxelNet&Swin-T&- & - & \textbf{62.3} &-\\
%          \midrule
%           \midrule
%          \multicolumn{9}{c}{3D Detection + BEV Map Segmentation}\\
%           \midrule
%          BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (share) & C+L  &0.1 & VoxelNet&Swin-T & - &  69.7 &  54.0 &-\\
%          BEVFusion$^{\dag}$~\cite{liu2022bevfusion} (sep) & C+L  &0.1 &VoxelNet&Swin-T &  - &  69.9 &  58.4 &-\\
%          % Baseline$^{*}$ (upper bound) &C+L &D+S & 62.07 & 66.57 & 62.27\\
%          % Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T& \cellcolor{blue!5}\textbf{59.09} & \cellcolor{blue!5}\textbf{65.03} & \cellcolor{blue!5}\textbf{43.97}\\
%          % Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T &\cellcolor{blue!5}\textbf{60.47} &\cellcolor{blue!5}\textbf{65.34}  &\cellcolor{blue!5}\textbf{58.35}\\
%          Baseline(share)& C+L  &0.1 &VoxelNet&Swin-T&  {59.1} &  {65.0} &  {44.0} & {33.6}\\
%          Fuller(share) &C+L  &0.1 & VoxelNet&Swin-T & \textbf{60.5} & \textbf{65.3}  & \textbf{58.4} & \textbf{10.8}\\
%          \bottomrule
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[$\dag$] means the multi-task result in BEVFusion\cite{liu2022bevfusion}. $^{\ddag}$ means re-implementation result in BEVFusion\cite{liu2022bevfusion}. `share' means multi-task heads share one BEV encoder to process the fused multimodal feature. `sep' means task heads have separate encoders.
%     \end{tablenotes}
% \end{threeparttable}}
% \vspace{-3mm}
% \label{tab:baseline}
% \end{table*}

==> tab/mtl_result.tex <==
% \begin{table}
%   \centering
%   \caption{
%   % \xd{move to experiment as we have many analysis figures before method already} 
%   % We evaluate existing works of multi-task learning in our baseline. We empirically find that GradNorm and xx, though is able to reduce the discrepancy of gradient magnitude, are unfavorable to our model. IMTL can alleviate the task conflict considerably. We conjecture that this is because IMTL also attends the gradient direction. 
%   We qualitatively and quantitatively evaluate existing works of multi-task learning in our baseline. They are able to reduce the discrepancy of gradient magnitude and improve the subsequent performance. Throughout the paper, IMTL is adopted as the technique for inter-gradient calibration.\xd{list the average number of multi-task in table}
%   }
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{3pt}{1.0}
%   \begin{tabular}{@{}lccccc@{}}
%     \toprule
%     Method & $\gamma_{\rm task}$ &mAP(\%) & NDS &mIoU(\%) &$\Delta_{\rm MTL}$\\
%     \midrule
%     Baseline  &16.87 & 59.09 &65.03 &43.90 &-\\
%     GradNorm~\cite{chen2018gradnorm}  &12.54 & 58.33 & 64.41 & 57.19&\\
%     DWA~\cite{liu2019end} &-  &\textbf{59.29} & \textbf{65.14} & 57.72 &\\
%     IMTL~\cite{liu2021towards} &1.07  &57.07 &63.34  &\textbf{59.40} &\\
%     \bottomrule
%   \end{tabular}}
%   \label{tab:mtl_result}
% \end{table}


% \begin{table}
%   \centering
%   \caption{
%   We qualitatively and quantitatively evaluate existing works of multi-task learning in our baseline. They are able to reduce the discrepancy of gradient magnitude and improve the subsequent performance. 
%   \lsh{Note that DWA has to..}
%   % Throughout the paper, IMTL is adopted as the technique for inter-gradient calibration.
%   }\vspace{-4mm}
%     \resizebox{1.0\columnwidth}{!}
%     {\tablestyle{5pt}{1.0}
%   \begin{tabular}{@{}lccccc@{}}
%     \toprule
%     Method & $\gamma_{\rm task}$ $^\downarrow$ &mAP(\%)$^\uparrow$ 
%     & NDS$^\uparrow$ &mIoU(\%)$^\uparrow$ &$\Delta_{\rm MTL}$(\%) $^\downarrow$\\
%     \midrule
%     Baseline  &16.87 & 59.1 &65.0 &44.0 &36.6\\
%     GradNorm~\cite{chen2018gradnorm}  &12.54 & 58.3 & 64.4 & 57.2&17.6\\
%     DWA~\cite{liu2019end} &-  &59.3 & 65.1 & 57.7 &14.1\\
%     IMTL\_G~\cite{liu2021towards} &1.13  &57.1 &63.3 &\textbf{59.4} &17.7\\
%     \midrule
%     Fuller (Ours) &1.07 &\textbf{60.5} &\textbf{65.3} &58.4 &\textbf{10.8} \\
    
%     \bottomrule
%   \end{tabular}}
%   \label{tab:mtl_result}
% \end{table}

\begin{table}
  \centering
  % \caption{We compare existing works of multi-task learning.}
  \caption{DWA needs to empirically select the initial loss weights while GradNorm uses extra learnable parameters. Considering scalability and performance, we select the IMTL\_G as the inter-gradient calibration.}
  \vspace{-0mm}
  \resizebox{1.0\columnwidth}{!}
  {\tablestyle{8pt}{1.0}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Method &mAP(\%)$\uparrow$ 
    & NDS$\uparrow$ &mIoU(\%)$\uparrow$ &$\Delta_{\rm MTL}$(\%) $\downarrow$\\
    \midrule
    Baseline  & 59.1 &65.0 &44.0 &36.6\\
    GradNorm~\cite{chen2018gradnorm}  & 58.3 & 64.4 & 57.2&17.6\\
    DWA~\cite{liu2019end}  &59.3 & 65.1 & 57.7 &14.1\\
    IMTL\_G~\cite{liu2021towards}  &57.1 &63.3 &\textbf{59.4} &17.7\\
    \midrule
    Fuller (Ours) &\textbf{60.5} &\textbf{65.3} &58.4 &\textbf{10.8} \\
    
    \bottomrule
  \end{tabular}}
  \label{tab:mtl_result}
\end{table}

==> tab/relation_inter_intra.tex <==
\begin{table}[t]
  \centering
  \vspace{-1mm}
  \caption{
  Relation between inter- and intra-gradient calibration.
  }\vspace{-0mm}
\resizebox{0.9\columnwidth}{!}
{\tablestyle{12pt}{1.0}
  \begin{tabular}{@{}cc|ccc@{}}
    \toprule
        Intra. & Inter. &$\gamma_{\rm task}$$\downarrow$ 
        &$\gamma_{\rm modal}$$\downarrow$ &$\Delta_{\rm MTL}$ $\downarrow$\\
        \midrule
        & &19.2 &3.7 &18.3 \\
        \checkmark & &12.5 &1.9 &16.9 \\
         &\checkmark &2.5  &2.8 &8.8 \\
        \checkmark &\checkmark &\textbf{1.9}  &\textbf{1.7} &\textbf{5.4} \\
\bottomrule
    \end{tabular}}
  \label{tab:relation_inter_intra}
  \vspace{-4mm}
\end{table}

==> tab/task_head.tex <==
\begin{table}[!t]
  \centering
  \vspace{-1mm}
  \caption{
  Comparison between task heads.  %\gy{running experiment under 0.1 voxel size }
  }\vspace{-0mm}
\resizebox{1.0\columnwidth}{!}
{\tablestyle{10pt}{1.0}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Method  
    &mAP(\%)$\uparrow$
    & NDS$\uparrow
    $&mIoU(\%)$\uparrow$ & Params$\downarrow$\\
    \midrule
    CenterPoint\cite{yin2021center}  &58.6  & 64.8  &- & 1.6m \\
    Fuller-det (Ours) & \textbf{62.1} & \textbf{66.6} & - & \textbf{1.0m} \\
    BEVFusion\cite{liu2022bevfusion} & - & - &  \textbf{62.7} & 4.7m \\
    Fuller-seg (Ours) & - & - & 62.3 & \textbf{2.7m}\\

    \bottomrule
  \end{tabular}}\vspace{-2mm}
  \label{tab:task_head}
\end{table}
